Test Case-Informed Knowledge Tracing for Open-ended Coding Tasks

Open-ended coding tasks, which ask students to construct programs according to certain specifications, are common in computer science education. Student modeling can be challenging since their open-ended nature means that student code can be diverse. Traditional knowledge tracing (KT) models that only analyze response correctness may not fully capture nuances in student knowledge from student code. In this paper, we introduce Test case-Informed Knowledge Tracing for Open-ended Coding (TIKTOC), a framework to simultaneously analyze and predict both open-ended student code and whether the code passes each test case. We augment the existing CodeWorkout dataset with the test cases used for a subset of the open-ended coding questions, and propose a multi-task learning KT method to simultaneously analyze and predict 1) whether a student's code submission passes each test case and 2) the student's open-ended code, using a large language model as the backbone. We quantitatively show that these methods outperform existing KT methods for coding that only use the overall score a code submission receives. We also qualitatively demonstrate how test case information, combined with open-ended code, helps us gain fine-grained insights into student knowledge.

==> student_codes/conciseness_11.tex <==
\begin{lstlisting}
public int caughtSpeeding(int speed, boolean isBirthday)
{
    if (isBirthday)
        if (speed <= 65)
            return 0;
        else if (speed >= 66 && speed <= 85)
            return 1;
        else
            return 2;
    else
        if (speed <= 60)
            return 0;
        else if (speed >= 61 && speed <= 80)
            return 1;
        else
            return 2;
}\end{lstlisting}

==> student_codes/conciseness_12.tex <==
\begin{lstlisting}
public int caughtSpeeding(int speed, boolean isBirthday)
{
    if(isBirthday)
        speed -= 5;
    if(speed <= 60)
        return 0;
    else if(speed <= 80)
        return 1;
    else
        return 2;
}\end{lstlisting}

==> student_codes/conciseness_41.tex <==
\begin{lstlisting}
public boolean cigarParty(int cigars, boolean isWeekend)
{
    if (isWeekend)
        if (cigars >= 40)
            return true;
        else
            return false;
    else
        if (cigars >= 40 && cigars <= 60)
            return true;
        else
            return false;
}\end{lstlisting}

==> student_codes/conciseness_42.tex <==
\begin{lstlisting}
public boolean cigarParty(int cigars, boolean isWeekend)
{
    if(isWeekend)
        return (cigars >= 40);
    return (cigars >= 40 && cigars <= 60);
}\end{lstlisting}
